CC2Vec: Distributed Representations of Code Changes

Existing work on software patches often use features specific to a single task. These works often rely on manually identified features, and human effort is required to identify these features for each task. In this work, we propose CC2Vec, a neural network model that learns a representation of code changes guided by their accompanying log messages, which represent the semantic intent of the code changes. CC2Vec models the hierarchical structure of a code change with the help of the attention mechanism and uses multiple comparison functions to identify the differences between the removed and added code. To evaluate if CC2Vec can produce a distributed representation of code changes that is general and useful for multiple tasks on software patches, we use the vectors produced by CC2Vec for three tasks: log message generation, bug fixing patch identification, and just-in-time defect prediction. In all tasks, the models using CC2Vec outperform the state-of-the-art techniques.

==> bib.tex <==
@article{hoang2019patchnet,
  title={PatchNet: Hierarchical Deep Learning-Based Stable Patch Identification for the Linux Kernel},
  author={Hoang, Thong and Lawall, Julia and Tian, Yuan and Oentaryo, Richard J and Lo, David},
  journal={IEEE Transactions on Software Engineering},
  year={2019},
  publisher={IEEE}
}

@inproceedings{wang2017compare,
  author    = {Shuohang Wang and
               Jing Jiang},
  title     = {A Compare-Aggregate Model for Matching Text Sequences},
  booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
               Toulon, France, April 24-26, 2017, Conference Track Proceedings},
  year      = {2017},
  url       = {https://openreview.net/forum?id=HJTzHtqee},
  timestamp = {Thu, 25 Jul 2019 14:25:54 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iclr/Wang017},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@incollection{nguyen2009learning,
  title={Learning pattern classification tasks with imbalanced data sets},
  author={Nguyen, Giang Hoang and Bouzerdoum, Abdesselam and Phung, Son Lam},
  booktitle={Pattern recognition},
  year={2009},
  publisher={IntechOpen}
}

@inproceedings{kim2014convolutional,
    title = "Convolutional Neural Networks for Sentence Classification",
    author = "Kim, Yoon",
    booktitle = "Proceedings of the 2014 Conference on Empirical Methods in Natural Language Processing ({EMNLP})",
    month = oct,
    year = "2014",
    address = "Doha, Qatar",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/D14-1181",
    doi = "10.3115/v1/D14-1181",
    pages = "1746--1751",
}

@article{joachims1999svmlight,
  title={Svmlight: Support vector machine},
  author={Joachims, Thorsten},
  journal={SVM-Light Support Vector Machine http://svmlight. joachims. org/, University of Dortmund},
  volume={19},
  number={4},
  year={1999}
}

@inproceedings{lee2003learning,
  title={Learning with positive and unlabeled examples using weighted logistic regression},
  author={Lee, Wee Sun and Liu, Bing},
  booktitle={ICML},
  volume={3},
  pages={448--455},
  year={2003}
}

@inproceedings{papineni2002bleu,
  title={BLEU: a method for automatic evaluation of machine translation},
  author={Papineni, Kishore and Roukos, Salim and Ward, Todd and Zhu, Wei-Jing},
  booktitle={Proceedings of the 40th annual meeting on association for computational linguistics},
  pages={311--318},
  year={2002},
  organization={Association for Computational Linguistics}
}

@article{manning2010introduction,
  title={Introduction to information retrieval},
  author={Manning, Christopher and Raghavan, Prabhakar and Sch{\"u}tze, Hinrich},
  journal={Natural Language Engineering},
  volume={16},
  number={1},
  pages={100--103},
  year={2010},
  publisher={Cambridge university press}
}

@inproceedings{linares2015changescribe,
  title={Changescribe: A tool for automatically generating commit messages},
  author={Linares-V{\'a}squez, Mario and Cort{\'e}s-Coy, Luis Fernando and Aponte, Jairo and Poshyvanyk, Denys},
  booktitle={2015 IEEE/ACM 37th IEEE International Conference on Software Engineering},
  volume={2},
  pages={709--712},
  year={2015},
  organization={IEEE}
}

@inproceedings{yang2016hierarchical,
  title={Hierarchical attention networks for document classification},
  author={Yang, Zichao and Yang, Diyi and Dyer, Chris and He, Xiaodong and Smola, Alex and Hovy, Eduard},
  booktitle={Proceedings of the 2016 conference of the North American chapter of the association for computational linguistics: human language technologies},
  pages={1480--1489},
  year={2016}
}

@article{danielsson1980euclidean,
  title={Euclidean distance mapping},
  author={Danielsson, Per-Erik},
  journal={Computer Graphics and image processing},
  volume={14},
  number={3},
  pages={227--248},
  year={1980},
  publisher={Elsevier}
}

@article{hagan1994training,
  title={Training feedforward networks with the Marquardt algorithm},
  author={Hagan, Martin T and Menhaj, Mohammad B},
  journal={IEEE transactions on Neural Networks},
  volume={5},
  number={6},
  pages={989--993},
  year={1994},
  publisher={IEEE}
}

@article{arora2018optimization,
  title={On the optimization of deep networks: Implicit acceleration by overparameterization},
  author={Arora, Sanjeev and Cohen, Nadav and Hazan, Elad},
  journal={arXiv preprint arXiv:1802.06509},
  year={2018}
}

@article{anthimopoulos2016lung,
  title={Lung pattern classification for interstitial lung diseases using a deep convolutional neural network},
  author={Anthimopoulos, Marios and Christodoulidis, Stergios and Ebner, Lukas and Christe, Andreas and Mougiakakou, Stavroula},
  journal={IEEE transactions on medical imaging},
  volume={35},
  number={5},
  pages={1207--1216},
  year={2016},
  publisher={IEEE}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@article{srivastava2014dropout,
  title={Dropout: a simple way to prevent neural networks from overfitting},
  author={Srivastava, Nitish and Hinton, Geoffrey and Krizhevsky, Alex and Sutskever, Ilya and Salakhutdinov, Ruslan},
  journal={The Journal of Machine Learning Research},
  volume={15},
  number={1},
  pages={1929--1958},
  year={2014},
  publisher={JMLR. org}
}

@inproceedings{caruana2001overfitting,
  title={Overfitting in neural nets: Backpropagation, conjugate gradient, and early stopping},
  author={Caruana, Rich and Lawrence, Steve and Giles, C Lee},
  booktitle={Advances in neural information processing systems},
  pages={402--408},
  year={2001}
}

@article{svozil1997introduction,
  title={Introduction to multi-layer feed-forward neural networks},
  author={Svozil, Daniel and Kvasnicka, Vladimir and Pospichal, Jiri},
  journal={Chemometrics and intelligent laboratory systems},
  volume={39},
  number={1},
  pages={43--62},
  year={1997},
  publisher={Elsevier}
}

@inproceedings{bai2018deep,
  title={Deep attention neural tensor network for visual question answering},
  author={Bai, Yalong and Fu, Jianlong and Zhao, Tiejun and Mei, Tao},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={20--35},
  year={2018}
}

@inproceedings{qiu2015convolutional,
  title={Convolutional neural tensor network architecture for community-based question answering},
  author={Qiu, Xipeng and Huang, Xuanjing},
  booktitle={Twenty-Fourth International Joint Conference on Artificial Intelligence},
  year={2015}
}

@inproceedings{socher2013recursive,
  title={Recursive deep models for semantic compositionality over a sentiment treebank},
  author={Socher, Richard and Perelygin, Alex and Wu, Jean and Chuang, Jason and Manning, Christopher D and Ng, Andrew and Potts, Christopher},
  booktitle={Proceedings of the 2013 conference on empirical methods in natural language processing},
  pages={1631--1642},
  year={2013}
}

@inproceedings{bouchard2007efficient,
  title={Efficient bounds for the softmax function and applications to approximate inference in hybrid models},
  author={Bouchard, Guillaume},
  booktitle={NIPS 2007 workshop for approximate Bayesian inference in continuous/hybrid systems},
  year={2007}
}

@inproceedings{kumar2016ask,
  title={Ask me anything: Dynamic memory networks for natural language processing},
  author={Kumar, Ankit and Irsoy, Ozan and Ondruska, Peter and Iyyer, Mohit and Bradbury, James and Gulrajani, Ishaan and Zhong, Victor and Paulus, Romain and Socher, Richard},
  booktitle={International conference on machine learning},
  pages={1378--1387},
  year={2016}
}

@inproceedings{sukhbaatar2015end,
  title={End-to-end memory networks},
  author={Sukhbaatar, Sainbayar and Weston, Jason and Fergus, Rob and others},
  booktitle={Advances in neural information processing systems},
  pages={2440--2448},
  year={2015}
}

@article{anastassiou2011univariate,
  title={Univariate hyperbolic tangent neural network approximation},
  author={Anastassiou, George A},
  journal={Mathematical and Computer Modelling},
  volume={53},
  number={5-6},
  pages={1111--1132},
  year={2011},
  publisher={Elsevier}
}

@inproceedings{dahl2013improving,
  title={Improving deep neural networks for LVCSR using rectified linear units and dropout},
  author={Dahl, George E and Sainath, Tara N and Hinton, Geoffrey E},
  booktitle={2013 IEEE international conference on acoustics, speech and signal processing},
  pages={8609--8613},
  year={2013},
  organization={IEEE}
}

@inproceedings{nair2010rectified,
  title={Rectified linear units improve restricted boltzmann machines},
  author={Nair, Vinod and Hinton, Geoffrey E},
  booktitle={Proceedings of the 27th international conference on machine learning (ICML-10)},
  pages={807--814},
  year={2010}
}

@article{bahdanau2014neural,
	title={Neural machine translation by jointly learning to align and translate},
	author={Bahdanau, Dzmitry and Cho, Kyunghyun and Bengio, Yoshua},
	journal={arXiv preprint arXiv:1409.0473},
	year={2014}
}

@inproceedings{socher2013reasoning,
	title={Reasoning with neural tensor networks for knowledge base completion},
	author={Socher, Richard and Chen, Danqi and Manning, Christopher D and Ng, Andrew},
	booktitle={Advances in neural information processing systems},
	pages={926--934},
	year={2013}
}

@article{gunther2010neuralnet,
	title={neuralnet: Training of neural networks},
	author={G{\"u}nther, Frauke and Fritsch, Stefan},
	journal={The R journal},
	volume={2},
	number={1},
	pages={30--38},
	year={2010}
}

@inproceedings{cheung2012convolutional,
	title={Convolutional neural networks applied to human face classification},
	author={Cheung, Brian},
	booktitle={2012 11th International Conference on Machine Learning and Applications},
	volume={2},
	pages={580--583},
	year={2012},
	organization={IEEE}
}

@inproceedings{maji2011action,
	title={Action recognition from a distributed representation of pose and appearance},
	author={Maji, Subhransu and Bourdev, Lubomir and Malik, Jitendra},
	booktitle={CVPR 2011},
	pages={3177--3184},
	year={2011},
	organization={IEEE}
}

@inproceedings{mikolov2013distributed,
	title={Distributed representations of words and phrases and their compositionality},
	author={Mikolov, Tomas and Sutskever, Ilya and Chen, Kai and Corrado, Greg S and Dean, Jeff},
	booktitle={Advances in neural information processing systems},
	pages={3111--3119},
	year={2013}
}

@inproceedings{rahman2015textrank,
	title={TextRank based search term identification for software change tasks},
	author={Rahman, Mohammad Masudur and Roy, Chanchal K},
	booktitle={2015 IEEE 22nd International Conference on Software Analysis, Evolution, and Reengineering (SANER)},
	pages={540--544},
	year={2015},
	organization={IEEE}
}

@inproceedings{liu2018neural,
	title={Neural-machine-translation-based commit message generation: how far are we?},
	author={Liu, Zhongxin and Xia, Xin and Hassan, Ahmed E and Lo, David and Xing, Zhenchang and Wang, Xinyu},
	booktitle={Proceedings of the 33rd ACM/IEEE International Conference on Automated Software Engineering},
	pages={373--384},
	year={2018},
	organization={ACM}
}

@inproceedings{bird2004nltk,
	title={NLTK: the natural language toolkit},
	author={Bird, Steven and Loper, Edward},
	booktitle={Proceedings of the ACL 2004 on Interactive poster and demonstration sessions},
	pages={31},
	year={2004},
	organization={Association for Computational Linguistics}
}

@article{ji20123d,
	title={3D convolutional neural networks for human action recognition},
	author={Ji, Shuiwang and Xu, Wei and Yang, Ming and Yu, Kai},
	journal={IEEE transactions on pattern analysis and machine intelligence},
	volume={35},
	number={1},
	pages={221--231},
	year={2012},
	publisher={IEEE}
}

@article{chapelle2009semi,
	title={Semi-supervised learning (chapelle, o. et al., eds.; 2006)[book reviews]},
	author={Chapelle, Olivier and Scholkopf, Bernhard and Zien, Alexander},
	journal={IEEE Transactions on Neural Networks},
	volume={20},
	number={3},
	pages={542--542},
	year={2009},
	publisher={IEEE}
}

@inproceedings{yang2015deep,
	title={Deep learning for just-in-time defect prediction},
	author={Yang, Xinli and Lo, David and Xia, Xin and Zhang, Yun and Sun, Jianling},
	booktitle={2015 IEEE International Conference on Software Quality, Reliability and Security},
	pages={17--26},
	year={2015},
	organization={IEEE}
}

@book{bishop2006pattern,
	title={Pattern recognition and machine learning},
	author={Bishop, Christopher M},
	year={2006},
	publisher={springer}
}

@article{kim2008classifying,
	title={Classifying software changes: Clean or buggy?},
	author={Kim, Sunghun and Whitehead Jr, E James and Zhang, Yi},
	journal={IEEE Transactions on Software Engineering},
	volume={34},
	number={2},
	pages={181--196},
	year={2008},
	publisher={IEEE}
}

@article{mockus2000predicting,
	title={Predicting risk of software changes},
	author={Mockus, Audris and Weiss, David M},
	journal={Bell Labs Technical Journal},
	volume={5},
	number={2},
	pages={169--180},
	year={2000},
	publisher={Wiley Online Library}
}

@inproceedings{tian2012identifying,
	title={Identifying Linux bug fixing patches},
	author={Tian, Yuan and Lawall, Julia and Lo, David},
	booktitle={Proceedings of the 34th International Conference on Software Engineering},
	pages={386--396},
	year={2012},
	organization={IEEE Press}
}

@inproceedings{hoang2019deepjit,
	title={DeepJIT: an end-to-end deep learning framework for just-in-time defect prediction},
	author={Hoang, Thong and Dam, Hoa Khanh and Kamei, Yasutaka and Lo, David and Ubayashi, Naoyasu},
	booktitle={Proceedings of the 16th International Conference on Mining Software Repositories},
	pages={34--45},
	year={2019},
	organization={IEEE Press}
}

@inproceedings{rahman2016correct,
	title={Correct: code reviewer recommendation in github based on cross-project and technology experience},
	author={Rahman, Mohammad Masudur and Roy, Chanchal K and Collins, Jason A},
	booktitle={2016 IEEE/ACM 38th International Conference on Software Engineering Companion (ICSE-C)},
	pages={222--231},
	year={2016},
	organization={IEEE}
}

@inproceedings{kirinuki2014hey,
	title={Hey! are you committing tangled changes?},
	author={Kirinuki, Hiroyuki and Higo, Yoshiki and Hotta, Keisuke and Kusumoto, Shinji},
	booktitle={Proceedings of the 22nd International Conference on Program Comprehension},
	pages={262--265},
	year={2014},
	organization={ACM}
}

@article{kamei2016studying,
  title={Studying just-in-time defect prediction using cross-project models},
  author={Kamei, Yasutaka and Fukushima, Takafumi and McIntosh, Shane and Yamashita, Kazuhiro and Ubayashi, Naoyasu and Hassan, Ahmed E},
  journal={Empirical Software Engineering},
  volume={21},
  number={5},
  pages={2072--2106},
  year={2016},
  publisher={Springer}
}

@inproceedings{
    alon2018codeseq,
    title={code2seq: Generating Sequences from Structured Representations of Code},
    author={Uri Alon and Shaked Brody and Omer Levy and Eran Yahav},
    booktitle={International Conference on Learning Representations},
    year={2019}
}

@article{alon2019code2vec,
  title={code2vec: Learning distributed representations of code},
  author={Alon, Uri and Zilberstein, Meital and Levy, Omer and Yahav, Eran},
  journal={Proceedings of the ACM on Programming Languages},
  volume={3},
  number={POPL},
  pages={40},
  year={2019},
  publisher={ACM}
}

@inproceedings{hu2018deep,
  title={Deep code comment generation},
  author={Hu, Xing and Li, Ge and Xia, Xin and Lo, David and Jin, Zhi},
  booktitle={Proceedings of the 26th Conference on Program Comprehension},
  pages={200--210},
  year={2018},
  organization={ACM}
}

@inproceedings{beller2017oops,
  title={Oops, my tests broke the build: An explorative analysis of Travis CI with GitHub},
  author={Beller, Moritz and Gousios, Georgios and Zaidman, Andy},
  booktitle={2017 IEEE/ACM 14th International Conference on Mining Software Repositories (MSR)},
  pages={356--367},
  year={2017},
  organization={IEEE}
}

@inproceedings{iyer2016summarizing,
  title={Summarizing source code using a neural attention model},
  author={Iyer, Srinivasan and Konstas, Ioannis and Cheung, Alvin and Zettlemoyer, Luke},
  booktitle={Proceedings of the 54th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  pages={2073--2083},
  year={2016}
}

@article{allamanis2018survey,
  title={A survey of machine learning for big code and naturalness},
  author={Allamanis, Miltiadis and Barr, Earl T and Devanbu, Premkumar and Sutton, Charles},
  journal={ACM Computing Surveys (CSUR)},
  volume={51},
  number={4},
  pages={81},
  year={2018},
  publisher={ACM}
}

@article{chen2019literature,
  title={A Literature Study of Embeddings on Source Code},
  author={Chen, Zimin and Monperrus, Martin},
  journal={arXiv preprint arXiv:1904.03061},
  year={2019}
}

@inproceedings{jiang2017automatically,
  title={Automatically generating commit messages from diffs using neural machine translation},
  author={Jiang, Siyuan and Armaly, Ameer and McMillan, Collin},
  booktitle={Proceedings of the 32nd IEEE/ACM International Conference on Automated Software Engineering},
  pages={135--146},
  year={2017},
  organization={IEEE Press}
}



@article{kamei2012large,
  title={A large-scale empirical study of just-in-time quality assurance},
  author={Kamei, Yasutaka and Shihab, Emad and Adams, Bram and Hassan, Ahmed E and Mockus, Audris and Sinha, Anand and Ubayashi, Naoyasu},
  journal={IEEE Transactions on Software Engineering},
  volume={39},
  number={6},
  pages={757--773},
  year={2012},
  publisher={IEEE}
}

@inproceedings{aversano2007learning,
  title={Learning from bug-introducing changes to prevent fault prone code},
  author={Aversano, Lerina and Cerulo, Luigi and Del Grosso, Concettina},
  booktitle={Ninth international workshop on Principles of software evolution: in conjunction with the 6th ESEC/FSE joint meeting},
  pages={19--26},
  year={2007},
  organization={ACM}
}




@inproceedings{dyer2013boa,
  title={Boa: A language and infrastructure for analyzing ultra-large-scale software repositories},
  author={Dyer, Robert and Nguyen, Hoan Anh and Rajan, Hridesh and Nguyen, Tien N},
  booktitle={Proceedings of the 2013 International Conference on Software Engineering},
  pages={422--431},
  year={2013},
  organization={IEEE Press}
}

@inproceedings{shihab2012industrial,
  title={An industrial study on the risk of software changes},
  author={Shihab, Emad and Hassan, Ahmed E and Adams, Bram and Jiang, Zhen Ming},
  booktitle={Proceedings of the ACM SIGSOFT 20th International Symposium on the Foundations of Software Engineering},
  pages={62},
  year={2012},
  organization={ACM}
}

@inproceedings{tantithamthavorn2015impact,
  title={The impact of mislabelling on the performance and interpretation of defect prediction models},
  author={Tantithamthavorn, Chakkrit and McIntosh, Shane and Hassan, Ahmed E and Ihara, Akinori and Matsumoto, Kenichi},
  booktitle={2015 IEEE/ACM 37th IEEE International Conference on Software Engineering},
  volume={1},
  pages={812--823},
  year={2015},
  organization={IEEE}
}

@article{mcintosh2017fix,
  title={Are fix-inducing changes a moving target? a longitudinal case study of just-in-time defect prediction},
  author={McIntosh, Shane and Kamei, Yasutaka},
  journal={IEEE Transactions on Software Engineering},
  volume={44},
  number={5},
  pages={412--428},
  year={2017},
  publisher={IEEE}
}

@inproceedings{gu2018deep,
  title={Deep code search},
  author={Gu, Xiaodong and Zhang, Hongyu and Kim, Sunghun},
  booktitle={2018 IEEE/ACM 40th International Conference on Software Engineering (ICSE)},
  pages={933--944},
  year={2018},
  organization={IEEE}
}

@inproceedings{xu2017answerbot,
  title={AnswerBot: automated generation of answer summary to developers{\'z} technical questions},
  author={Xu, Bowen and Xing, Zhenchang and Xia, Xin and Lo, David},
  booktitle={Proceedings of the 32nd IEEE/ACM International Conference on Automated Software Engineering},
  pages={706--716},
  year={2017},
  organization={IEEE Press}
}


@article{maaten2008visualizing,
  title={Visualizing data using t-SNE},
  author={Maaten, Laurens van der and Hinton, Geoffrey},
  journal={Journal of machine learning research},
  volume={9},
  number={Nov},
  pages={2579--2605},
  year={2008}
}

@inproceedings{leclair2019neural,
  title={A neural model for generating natural language summaries of program subroutines},
  author={LeClair, Alexander and Jiang, Siyuan and McMillan, Collin},
  booktitle={Proceedings of the 41st International Conference on Software Engineering},
  pages={795--806},
  year={2019},
  organization={IEEE Press}
}

@article{DBLP:conf/iclr/KimDHR17,
  title={Structured attention networks},
  author={Kim, Yoon and Denton, Carl and Hoang, Luong and Rush, Alexander M},
  journal={arXiv preprint arXiv:1702.00887},
  year={2017}
}

@inproceedings{kovalenko2019pathminer,
  title={PathMiner: a library for mining of path-based representations of code},
  author={Kovalenko, Vladimir and Bogomolov, Egor and Bryksin, Timofey and Bacchelli, Alberto},
  booktitle={Proceedings of the 16th International Conference on Mining Software Repositories},
  pages={13--17},
  year={2019},
  organization={IEEE Press}
}

@inproceedings{efstathiou2019semantic,
  title={Semantic source code models using identifier embeddings},
  author={Efstathiou, Vasiliki and Spinellis, Diomidis},
  booktitle={Proceedings of the 16th International Conference on Mining Software Repositories},
  pages={29--33},
  year={2019},
  organization={IEEE Press}
}

@inproceedings{theeten2019import2vec,
  title={Import2vec learning embeddings for software libraries},
  author={Theeten, Bart and Vandeputte, Frederik and Van Cutsem, Tom},
  booktitle={Proceedings of the 16th International Conference on Mining Software Repositories},
  pages={18--28},
  year={2019},
  organization={IEEE Press}
}

@inproceedings{yin2018learning,
  title={Learning to mine aligned code and natural language pairs from stack overflow},
  author={Yin, Pengcheng and Deng, Bowen and Chen, Edgar and Vasilescu, Bogdan and Neubig, Graham},
  booktitle={2018 IEEE/ACM 15th International Conference on Mining Software Repositories (MSR)},
  pages={476--486},
  year={2018},
  organization={IEEE}
}


@inproceedings{nguyen2016mapping,
  title={Mapping API elements for code migration with vector representations},
  author={Nguyen, Trong Duc and Nguyen, Anh Tuan and Nguyen, Tien N},
  booktitle={2016 IEEE/ACM 38th International Conference on Software Engineering Companion (ICSE-C)},
  pages={756--758},
  year={2016},
  organization={IEEE}
}

@inproceedings{nguyen2017exploring,
  title={Exploring API embedding for API usages and applications},
  author={Nguyen, Trong Duc and Nguyen, Anh Tuan and Phan, Hung Dang and Nguyen, Tien N},
  booktitle={2017 IEEE/ACM 39th International Conference on Software Engineering (ICSE)},
  pages={438--449},
  year={2017},
  organization={IEEE}
}

@inproceedings{defreez2018path,
  title={Path-based function embedding and its application to error-handling specification mining},
  author={DeFreez, Daniel and Thakur, Aditya V and Rubio-Gonz{\'a}lez, Cindy},
  booktitle={Proceedings of the 2018 26th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering},
  pages={423--433},
  year={2018},
  organization={ACM}
}

@inproceedings{henkel2018code,
  title={Code vectors: Understanding programs through embedded abstracted symbolic traces},
  author={Henkel, Jordan and Lahiri, Shuvendu K and Liblit, Ben and Reps, Thomas},
  booktitle={Proceedings of the 2018 26th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering},
  pages={163--174},
  year={2018},
  organization={ACM}
}

@article{wang2017dynamic,
  title={Dynamic neural program embedding for program repair},
  author={Wang, Ke and Singh, Rishabh and Su, Zhendong},
  journal={arXiv preprint arXiv:1711.07163},
  year={2017}
}


